Constraining kaon PDFs from Drell-Yan and $J/\psi$ production

The kaon parton distribution functions (PDFs) are poorly known due to paucity of kaon-induced Drell-Yan data. Nevertheless, these Drell-Yan data suggest a softer valence $u$ quark distribution of kaon than that of pion. We discuss the opportunity to constrain kaon PDFs utilizing existing kaon-induced $J/\psi$ production data. We compare the $K^- / \pi^-$ and $K^+ / \pi^+$ cross-section ratio data with calculations based on two global-fit parametrizations and two recent theoretical predictions for the kaon and pion PDFs, and test the results with two quarkonium production models. The $K^- / \pi^-$ cross-section ratio for $J/\psi$ production provides independent evidence of different valence quark distributions in pion and kaon. The $K^+ / \pi^+$ $J/\psi$ data are found to be sensitive to the gluon distribution in kaon. We show that these $J/\psi$ production data provide valuable constraints for evaluating the adequacy of currently available sets of kaon PDFs.

==> ref.tex <==
\begin{thebibliography}{99}

\bibitem{Lin:2020ssv}
\cred{H.~W.~Lin, J.~W.~Chen, Z.~Fan, J.~H.~Zhang and R.~Zhang,
Valence-Quark Distribution of the Kaon and Pion from Lattice QCD,
Phys. Rev. D \textbf{103}, no.1, 014516 (2021).}
%[arXiv:2003.14128 [hep-lat]].

\bibitem{Fan:2021bcr}
\cred{Z.~Fan and H.~W.~Lin,
Gluon parton distribution of the pion from lattice QCD,
Phys. Lett. B \textbf{823}, 136778 (2021).}
%[arXiv:2104.06372 [hep-lat]].

\bibitem{Salas-Chavira:2021wui}
\cred{A.~Salas-Chavira, Z.~Fan and H.~W.~Lin,
First glimpse into the kaon gluon parton distribution using lattice QCD,
Phys. Rev. D \textbf{106}, 094510 (2022).}
%[arXiv:2112.03124 [hep-lat]].

\bibitem{Horn16} T. Horn and C. D. Roberts,
The pion: an enigma within the Standard Model,
J. Phys. G {\bf 43}, 073001 (2016).

\bibitem{Aguilar20} A. Aguilar {\it et al.}, 
Pion and kaon structure at the Electron-Ion Collider,
Eur. Phys. J A{\bf 55} (2019) 190.

\bibitem{DSE} Z. F. Cui {\it et al.}, Kaon and pion parton
distributions, Eur. Phys. J. C{\bf 80}, 1064 (2020).

\bibitem{Lan:2019rba}
\cred{J.~Lan, C.~Mondal, S.~Jia, X.~Zhao and J.~P.~Vary,
Pion and kaon parton distribution functions from basis light front quantization and QCD evolution,
Phys. Rev. D \textbf{101}, 034024 (2020).}

\bibitem{Han21} \cred{ C. Han, G. Xie, and X. Chen,
An analysis of parton distribution functions of the pion and
the kaon with the maximum entropy input,
Eur. Phys. J. C {\bf 81}, 302 (2021).}

\bibitem{Ji95} X. Ji, Breakup of hadron masses and the energy-momentum
tensor of QCD,
Phys. Rev. D {\bf 52}, 271 (1995).

\bibitem{Roberts21} C. Roberts, D. Richards, T. Horn, and
L. Chang, Insights into the emergence of mass from studies 
of pion and kaon structure, Prog. Part. Nucl. Phys. {\bf 120},
103883 (2021).

\bibitem{NA10DY} B. Betev {\it et al.}, NA10 Collaboration,
Differential cross-section of high-mass muon pairs produced by a 194
GeV/c $\pi^-$ beam on a tungsten target,
Z. Phys. C {\bf 28}, 9 (1985).

\bibitem{E326DY} H. B. Greenlee {\it et al.}, E326 Collaboration,
Production of massive muon pairs in $\pi^-$-nucleus collisions
Phys. Rev. Lett. {\bf 55}, 1555 (1985).

\bibitem{E615DY} J. S. Conway {\it et al.}, E615 Collaboration,
Experimental study of muon pairs produced by 252-GeV pions on tungsten,
Phys. Rev. D {\bf 39}, 92 (1989).

\bibitem{Owens}
  J.~F.~Owens,
$Q^2$-dependent parametrizations of pion parton distribution functions,
  Phys.\ Rev.\ D {\bf 30}, 943 (1984).

\bibitem{ABFKW}
  P.~Aurenche, R.~Baier, M.~Fontannaz, M.~N.~Kienzle-Focacci, and M.~Werlen,
The gluon content of the pion from high $p_T$ direct photon production,
  Phys.\ Lett.\ B {\bf 233}, 517 (1989).

\bibitem{GRV}
  M.~Gluck, E.~Reya, and A.~Vogt,
Pionic parton distributions,
  Z.\ Phys.\ C {\bf 53}, 651 (1992).

\bibitem{GRS} M. Gl\"{u}ck, E. Reya, and M. Stratmann,
Mesonic parton densities derived from constituent quark model 
constraints, Eur. Phys. J. {\bf C2}, 159 (1998).

\bibitem{SMRS}
  P.~J.~Sutton, A.~D.~Martin, R.~G.~Roberts, and W.~J.~Stirling,
Parton distributions for the pion extracted from Drell-Yan and prompt
photon experiments,
  Phys.\ Rev.\ D {\bf 45}, 2349 (1992).

\bibitem{Peng17} J.~C.~Peng, W.~C.~Chang, S.~Platchkov and T.~Sawada,
Valence Quark and Gluon Distributions of Kaon from $J/\psi$ Production,
[arXiv:1711.00839 [hep-ph]].

\bibitem{Chang20}
  W.~C.~Chang, J.~C.~Peng, S.~Platchkov, and T.~Sawada,
Constraining gluon density of pions at large $x$ by
pion-induced $J/\psi$ production,
  Phys. Rev. D {\bf 102}, 054024 (2020).

\bibitem{Hsieh21} C.~Y. Hsieh, Y.~S. Lian, W.~C. Chang, J.~C. Peng,
S.~Platchkov, and T.~Sawada,
NRQCD analysis of charmonium production with pion and proton beams
at fixed-target energies,
Chin. J. Phys. {\bf 73}, 13 (2021).

\bibitem{Chang23} W.~C. Chang, J.~C. Peng,
S.~Platchkov, and T.~Sawada,
Fixed-target charmonium production and pion parton distributions,
Phys. Rev. D {\bf 107}, 056008 (2023).

\bibitem{Bourrely22} C. Bourrely, W. C. Chang, and J. C. Peng,
Pion partonic distributions in a statistical model from pion-induced
Drell-Yan and $J/\psi$ production data,
Phys. Rev. D \textbf{105}, 076018 (2022).

\bibitem{NA3DY} J. Badier {\em et al.},
Measurement of the $K^- / \pi^-$ structure function ratio using the
Drell-Yan process, Phys. Lett. B {\bf 93}, 354 (1980).

\bibitem{NA3JPSI} J. Badier {\em et al.},
Experimental $J/\psi$ Hadronic Production from 150 to 280 GeV/c,
Z. Phys. C
{\bf 20}, 101 (1983).

\bibitem{WA39} M. J. Corden {\em et al.}, Experimental results on $J/\psi$
production by $\pi^\pm, K^\pm, p$ and $\bar p$ beams at 39.5 GeV,
Phys. Lett. B{\bf 96}, 411 (1980).

\bibitem{DYNNLO} S. Catani {\it et al.}, 
Vector Boson production at hadron colliders: A fully exclusive QCD 
calculation at Next-to-Next-to-Leading Order,
Phys. Rev. Lett. {\bf 103}, 082001 (2009).

\bibitem{EPPS16} K. J. Eskola, P. Paakkinen, H. Paukkunen, and
C. A. Salgado, EPPS16: nuclear parton distributions with LHC data,
Eur. Phys. J. C {\bf 77}, 163 (2017).

\bibitem{JAM} P. C. Barry, N. Sato, W. Melnitchouk, and C. R.
Ji, First Monte Carlo Global QCD Analysis of Pion Parton Distributions,
Phys. Rev. Lett. {\bf 121}, 152001 (2018).

\bibitem{Gavai} R. Gavai et al., Quarkonium production in hadronic collisions,
Int. J. Mod. Phys. A {\bf 10}, 3043
(1995).

\bibitem{Nelson} R. E. Nelson, R. Vogt, and A. D. Frawley, 
Narrowing the uncertainty on the total charm cross section and its 
effect on the $J/\psi$ cross section,
Phys. Rev. C {\bf 87}, 014908 (2013).

%\bibitem{Lansberg} J. P. Lansberg, H. S. Shao, N. Yamanaka,
%Y. J. Zhang, and C. Nous, 
%Complete NLO QCD study of single- and double-quarkonium hadroproduction 
%in the colour-evaporation model at the Tevatron and the LHC,
%Phys. Lett. B {\bf 807}, 135559 (2020).

\bibitem{Bodwin} G. T. Bodwin, E. Braaten, and G. P. Lepage,
Rigorous QCD analysis of inclusive annihilation and production of
heavy quarkonium, Phys. Rev. D {\bf 51}, 1125 (1995).

\bibitem{Beneke:1996tk}
\cred{M.~Beneke and I.~Z.~Rothstein,
Hadroproduction of quarkonia in fixed target experiments,
Phys. Rev. D \textbf{54}, 2005 (1996).}

\bibitem{Nason} P. Nason, S. Dawson, and R. K. Ellis, 
The total cross section for the production of heavy quarks 
in hadronic collisions, Nucl. Phys.
{\bf B303}, 607 (1988).

\bibitem{Mangano} M. L. Mangano, P. Nason, and G. Ridolfi, 
Fixed-target hadroproduction of heavy quarks, Nucl. Phys.
{\bf B405}, 507 (1993).

\bibitem{xFitter} I. Novikov {\it et al.}, 
Parton distribution functions of the charged pion within the 
xFitter framework,
Phys. Rev. D {\bf 102}, 014040 (2020). 

\bibitem{Londergan:1996vh}
J.~T. Londergan, G.~Q. Liu, A.~W. Thomas, {Kaon - nucleus Drell-Yan processes
  and kaon structure functions}, Phys. Lett. B380 (1996) 393--398.

\bibitem{AMBER} B.~Adams \textit{et al.}  Letter of Intent: A New QCD
  facility at the M2 beam line of the CERN SPS (COMPASS++/AMBER,
  [arXiv:1808.00848 [hep-ex]].

\bibitem{Claude24} C. Bourrely, F. Buccella, W. C. Chang, and J. C. Peng,
Extraction of kaon partonic distribution functions from the
Drell-Yan and $J/\psi$ production data,
Phys. Lett. B {\bf 848}, 138395 (2024).

\end{thebibliography}

